DeepGate: Learning Neural Representations of Logic Gates

Applying deep learning (DL) techniques in the electronic design automation (EDA) field has become a trending topic. Most solutions apply well-developed DL models to solve specific EDA problems. While demonstrating promising results, they require careful model tuning for every problem. The fundamental question on "How to obtain a general and effective neural representation of circuits?" has not been answered yet. In this work, we take the first step towards solving this problem. We propose DeepGate, a novel representation learning solution that effectively embeds both logic function and structural information of a circuit as vectors on each gate. Specifically, we propose transforming circuits into unified and-inverter graph format for learning and using signal probabilities as the supervision task in DeepGate. We then introduce a novel graph neural network that uses strong inductive biases in practical circuits as learning priors for signal probability prediction. Our experimental results show the efficacy and generalization capability of DeepGate.

==> dac22/conclusion.tex <==
%\subsection{Limitations and Future Work}

%Switching activity analysis is another crucial EDA task that can directly benefit from DeepGate. Here, we need to estimate the transition probabilities of each node in consecutive clock cycles. To accommodate this problem, we plan to add the transition probabilities (i.e., from logic ‘0’ to logic ‘1’ or vice versa) as supervision of separately-trained FCNs, which take the node embedding and the transition probabilities of its fan-in nodes as input features when finetuning the model


%We plan to apply the DeepGate-based SAT solver on some long-standing EDA tasks, such as equivalence checking in formal verification [52], [53], automatic test pattern generation (ATPG) [54]–[56], and logic optimization [57], [58]

\vspace{5pt}
\section{Conclusion and Future Work}
\label{sec:conclusion}
\vspace{5pt}


This paper proposes DeepGate, a novel representation learning solution that effectively embeds both logic functions and structural information of a circuit as vectors on each gate. In DeepGate, we construct easy-to-learn circuit graphs by transforming circuits into unified AIG format and introduce a novel GNN model with circuit knowledge as priors for effective representation learning. Using informative signal probability as supervision tasks on small sub-circuits, we show DeepGate can generalize to large circuits with accurate predictions without any pre-computed features.

While showing promising results, the current DeepGate model is still in its infancy. For example, we could introduce other informative supervision tasks (e.g., logic inference and Boolean satisfiability) to achieve better representations for logic gates. We could also add more circuits for training to build a large-scale foundation model for logic circuits~\cite{bommasani2021opportunities}. Moreover, in our future work, we plan to apply the representations learned in DeepGate onto many downstream EDA tasks (e.g., power estimation, logic reduction, and equivalence checking). These tasks are directly related to signal probability analysis, and we believe DeepGate can achieve satisfactory results without much effort in finetuning the model.
%GNN model for learning neural representation of logic gates. To estimate the simulated probability of logic gates, DeepGate leverages the gate type information, as well as the circuit structure, and is able to achieve highly-accurate probability prediction. Our empirical results show that DeepGate outperforms existing solutions significantly. %At the same time, this paper investigates the application of DeepGate 
%for test point insertion and shows the promising results. We leave other possible EDA tasks for future work.

%We build a foundation model for learning a suitable representation for logic gates in circuits. There are few aspects that we consider to further improve in our future work. Currently, we train and evaluate DeepGate only on open-sourced benchmarks but we consider to include industrial circuits as well in our future work. We use logic simulated probabilities as node level supervision, future efforts in this direction is to explore the other possible kinds of supervisions such as circuit satisfiability (SAT) and logic inference  process in circuits. We will investigate how can we model the logic inference process in DeepGate and utilize the circuit satisfiability information as an alternative supervision. We also plan to extend our work by applying DeepGate on some potential down-stream tasks such as \textit{Logic Reduction, Switching activity analysis} \textit{SAT Problem}. These kinds of works depends upon the logic probabilities and pattern simulations. These works can directly benefit from \textit{DeepGate}, without much effort in finetuning the model.


==> dac22/experiment.tex <==
\vspace{10pt}
\section{Experiments}
\label{sec:experiment}
\vspace{10pt}


\subsection{Datasets}\label{sec:dataset}
\vspace{5pt}
% \begin{table}
% \centering
% \caption{The Statistics of Circuit Dataset}
% \label{Tab:TrainSet}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{llllll} 
% \toprule
% Benchmark & \#Subcircuits & \#Nodes & \#Levels & \#RC    & LL Diff~ ~  \\ 
% \hline
% EPFL      & 828           & 84.8    & 13.5     & 6.84\%  & 6.3         \\
% ITC99     & 7560          & 361.0   & 22.4     & 19.76\% & 7.3         \\
% IWLS      & 1281          & 267.0   & 17.5     & 15.63\% & 9.5         \\
% Opencores & 1155          & 186.7   & 11.85    & 10.99\% & 6.2         \\
% \bottomrule
% \end{tabular}}
% \end{table}

\begin{table}
\centering
\caption{The Statistics of Circuit Training Dataset}
\label{Tab:TrainSet}

\begin{tabular}{llll} 
\toprule
% Benchmark & \#Subcircuits & \#Nodes & \#Node Range & \#Levels & Level Range\\ 
% \midrule
% EPFL      & 828           & 84.8   & 52--341 & 13.5     & 4--17 \\
% ITC99     & 7,560          & 361.0 & 36--1,947  & 22.4  & 3--23   \\
% IWLS      & 1,281          & 267.0 & 41--2,268  & 17.5  & 5--24   \\
% Opencores & 1,155          & 186.7 & 51--3,214  & 11.85 & 4--18  \\
% \midrule
% \textbf{Total}   & \textbf{10,824} & \textbf{310.1} & \textbf{36--3,214} & \textbf{20.1} & \textbf{3--24} \\
Benchmark & \#Subcircuits & \#Node & \#Level\\ 
\midrule
EPFL      & 828          & [52--341]      & [4--17] \\
ITC99     & 7,560          & [36--1,947]    & [3--23]   \\
IWLS      & 1,281          & [41--2,268]   & [5--24]   \\
Opencores & 1,155          & [51--3,214]   & [4--18]  \\
\midrule
\textbf{Total}   & \textbf{10,824} & \textbf{[36--3,214]} & \textbf{[3--24]} \\
\bottomrule
\end{tabular}
%\vspace{-10pt}
\end{table}
We extract many sub-circuits from four circuit benchmark suites: ITC’99~\cite{ITC99}, IWLS’05~\cite{albrecht2005iwls}, EPFL~\cite{EPFLBenchmarks} and OpenCore~\cite{takeda2008opencore}, and follow the circuit data preparation flow described in Section~\ref{sec:data-pre} to transform all circuits into a unified AIG format. We conduct logic simulations with up to $100k$ random input patterns to obtain an accurate signal probability on every node.


Table~\ref{Tab:TrainSet} presents the statistics of the circuit dataset.
\#Subcircuits shows the total number of subcircuits extracted from each benchmark. As shown in the table, the constructed circuit dataset covers circuit sizes ranging from tens to thousands of nodes with different logic levels. Finally, there are 
%We merge all extracted circuits together (
$10,824$ circuits in total, and we create $90/10$ training/test splits for model training and evaluation.

\subsection{Evaluation Metric and Baselines}
%We use the L1 loss as the evaluation metric to measure the prediction error. It 
To evaluate the performance of different GNN models, we calculate the average value of the absolute differences between the simulated probability $y_v$ and the predicted $\hat{y}_v$ from DeepGate for all nodes $\mathcal{V}$ in the circuits, as shown in equation~\eqref{eq:loss}. The smaller the value is, the better the model performs.
\vspace{5pt}
\begin{equation}
    \label{eq:loss}
    Avg.~Prediction~Error = \frac{1}{N} \sum_{v\in\mathcal{V}}{\left| y_v - \hat{y}_v \right|}
\end{equation}
%As the main challenge in logic probability prediction is the existence of reconvergence structures with complex logic sharing, we also report the average L1 loss for those nodes with highest error values (we select Top 5\% nodes here), denoted as $L1_{5\%}$. When a model can produce better estimations for those "difficult-to-analyze" logic gates, $L1_{5\%}$ will be smaller accordingly. 

We consider three GNN models: GCN, DAG-ConvGNN, and DAG-RecGNN. \textit{GCN} model treats the circuit graphs as undirected graphs in representation learning. DAG-ConvGNN model follows the settings defined in Equation~\eqref{eq:dag-edge}. For DAG-RecGNN model, we adopt the same COMBINE function and the reversed propagation layer design in DeepGate, as depicted in Section~\ref{sec:model}. As for the GNN model in DeepGate, it contains additional attention mechanism and skip connection (SC).  Under every setting, we evaluate 4 different aggregator designs, which include representative works for DAG learning, i.e., Convolutional Sum (abbreviated as Conv. Sum)~\cite{selsam2018learning}, Attention~\cite{velikovi2017graph, thost2021directed}, GatedSum~\cite{zhang2019dvae} and DeepSet~\cite{amizadeh2018learning}. 
%Please note that, for the DAG-RecGNN models, we adopt the same COMBINE function and the reversed propagation layer design in DeepGate, as depicted in Section~\ref{sec:model}.%, except that DeepGate uses the attention mechanism and skip connection design for reconvergence structures.
%recurrent updating scheme proposed in DeepGate. %The DeepGate we proposed in this work refers to the combination of DAG-RecGNN and Attention.

In order to make the comparison fair, we instantiate all models with $d=64$ for the node hidden states $\mathbf{h}_v$ and design the other parameterized functions to have a similar number of tunable parameters. For DAG-RecGNNs and our DeepGate model, a forward layer is followed by a reversed layer, and $T=10$ iterations of message passing are performed to obtain the final embeddings. We choose $L=8$ in Equation~\eqref{eq:positional} for the skip connection setting. For training, all models are optimized for $60$ epochs using the ADAM optimizer with a learning rate of $1\times10^{-4}$. We use the topological batching technique introduced in~\cite{thost2021directed} to accelerate the training.

\begin{table}
\centering
\caption{The Performance Comparison of DeepGate with other GNN models for Logic Probability Prediction}
\label{Tab:Comparison}
\begin{tabular}{lcc} 
\hline
Model             & Aggregator                                       & Avg. Prediction Error  \\ 
\hline
GCN               & Conv. Sum                                        & 0.1386                 \\
                  & Attention                                        & 0.1840                 \\
                  & DeepSet                                          & 0.2541                 \\
                  & GatedSum                                         & 0.1995                 \\ 
\hline
DAG-ConvGNN       & Conv. Sum                                        & 0.2215                 \\
                  & Attention                                        & 0.2398                 \\
                  & DeepSet                                          & 0.2431                 \\
                  & GatedSum                                         & 0.2333                 \\ 
\hline
DAG-RecGNN        & Conv. Sum                                        & 0.0328                 \\
(T=10)            & DeepSet                                          & 0.0302                 \\
                  & GatedSum                                         & 0.0329                 \\ 
\hline
\textbf{DeepGate} & Attention w/o SC                                 & \textbf{0.0234 }       \\
(T=10)            & Attention w/ SC & \textbf{0.0204 }       \\
\hline
\end{tabular}
% \vspace{-10pt}
\end{table}

\subsection{Probability Prediction}~\label{sec:prob}
\subsubsection{Comparison of DeepGate with Baseline Solutions}
% \vspace{-5pt}

%We demonstrate the effectiveness of DeepGate in terms of the accuracy of probabilities prediction on test circuits. 
Table~\ref{Tab:Comparison} compares DeepGate with other baseline solutions in terms of prediction error. From this table, we have several observations: First, both GCN and DAG-ConvGNN are subject to poor performance for probability prediction, mainly due to their lack of ability to model the computational behaviours of circuits. For instance, the best GCN model, equipped with Conv. Sum, gives $0.1386$ of prediction error, which in turn is even higher than the worst performing model of DAG-RecGNN. Therefore, only by incorporating the logical ordering into the model design and conducting the propagation recurrently, will make the model perform well. It shows the advantage of DAG-RecGNN implementation with dedicated recurrent scheme and reversed layer design discussed in Section~\ref{sec:model} over simpler GNN architectures. 
Second, among all models, DeepGate with attention alone achieves significant prediction error reduction. It brings $22.76\%$ relative improvement compared with the best baseline solution, which is the DAG-RecGNN model equipped with DeepSet aggregator. Hence, using the dedicated attention mechanism benefits logic representation learning. 
Third, equipped with skip connection design, DeepGate can further reduce the prediction error from $0.0234$ to $0.0204$, which reveals the efficacy of introducing the reconvergence knowledge into the model design. To summarize, with only the gate type information and the connectivity between gates, DeepGate learns to predict highly-accurate probabilities for logic gates.

As we observe that DAG-RecRNN with DeepSet aggregator (abbreviated as \textit{DeepSet} for the following discussion) performs better than the other baselines, in later results, we only compare DeepGate (w/ skip connection) with it.
% Figure. C1 and DeepGate prediction for now.

% \begin{figure}[t!]
% 	\centering
% 	\includegraphics[width=0.8\linewidth]{dac22/figs/Result.pdf}
% 	\caption{Probability Prediction Comparison of DeepGate with DeepSet based DAG-RecGNN model}
% 	\label{FIG:Res}
% \end{figure}

% \vspace{10pt}
\subsubsection{Results on Large Circuits}%~\newline
% \vspace{-5pt}

Furthermore, we evaluate DeepGate on five circuit designs that are substantially larger than the circuits it saw during training. The circuit statistics and the prediction error of both DeepGate and DeepSet are shown in Table~\ref{Tab:large-comparison}. The number of gates in these designs is two orders of magnitude more than that of the training circuits. 

We can observe that DeepGate achieves similar prediction accuracy as that on small circuits, and it outperforms DeepSet in these large circuits by a large margin. Such results clearly demonstrate the generalization capability of DeepGate.  In particular, DeepGate achieves $73.56\%$ prediction error reduction on \textit{Arbiter}. 
% achieving $36.88\%$ of relative reduction on average. 
This is because, the Arbiter circuit is designed to accommodate access from multiple requests, and it contains repetitive logic units with many reconvergence structures. As DeepGate treats such structures as a first-class citizen in the GNN model, it can generate much more accurate predictions. 
% against other baselines. We conjecture this is due to the benefits of good logic representation learned from DeepGate.

%the local structures share similar patterns among different scales of circuits, which facilitates DeepGate to generalize to larger circuits.





% \subsubsection{Visualization of Model Predictions}
% To show more detailed results, we randomly sample one circuit from the test dataset and visualize the prediction of all nodes in the circuit ($y$-axis) with the ground truth ($x$-axis) in Figure X. If a model can produce more accurate predictions, then the visualized results will be closer to an identity function. The two sub-figures clearly show the advantage of DeepGate (Left) against DAG-RecGNN with DeepSet aggregator (Right). Similar phenomenon are also observed for other circuits and models. %But still, some outliars 

% \begin{figure}[t!]
% 	\centering
% 	\includegraphics[width=0.8\linewidth]{dac22/figs/L1_Loss.pdf}
% 	\caption{L1 loss with with different recurrence iterations $T$.}
% 	\label{FIG:iteration}
% \end{figure}




\begin{table}
\centering
\renewcommand\tabcolsep{2.0pt}
\caption{The Performance Comparison of DeepGate and DeepSet on Five Large Circuits}
\label{Tab:large-comparison}
\begin{tabular}{@{}llllll@{}}
\toprule
Design  & \#Nodes & Levels & DeepSet & DeepGate & Reduction \\ \midrule
Arbiter      & 23.7K   & 173    & 0.0277  & 0.0073   & 73.56\%   \\
Squarer      & 36.0K   & 373    & 0.0495  & 0.0346   & 30.16\%   \\
Multiplier      & 47.3K   & 521    & 0.0220  & 0.0159   & 27.94\%   \\
80386 Processor      & 13.2K   & 122    & 0.0534  & 0.0387   & 27.56\%   \\
Viper Processor      & 40.5K   & 133    & 0.0520  & 0.0389   & 25.18\%   \\  \bottomrule
\end{tabular}
\end{table}
\iffalse
\begin{table}
\centering
\caption{Impact Analysis of different components of DeepGate}
\begin{tabular}{lll} 
\hline
Component                                                                                             & \begin{tabular}[c]{@{}l@{}}L1 Difference between\\~Prediction and Supervision\end{tabular} & \begin{tabular}[c]{@{}l@{}}\% Improvement\\Over Baseline\end{tabular}  \\ 
\hline
\begin{tabular}[c]{@{}l@{}}Modified Attention \\Mechanism\end{tabular}                                &                                                                                            &                                                                        \\ 
\hline
Skip Connection                                                                                       &                                                                                            &                                                                        \\ 
\hline
\begin{tabular}[c]{@{}l@{}}Customized\\Reverse Layer\end{tabular}                                     &                                                                                            &                                                                        \\ 
\hline
\begin{tabular}[c]{@{}l@{}}Modified Attention \\Mechanism \& \\Customized\\Reverse Layer\end{tabular} &                                                                                            &                                                                        \\ 
\hline
\begin{tabular}[c]{@{}l@{}}Skip Connection \& \\Customized\\Reverse Layer\end{tabular}                &                                                                                            &                                                                        \\
\hline
\end{tabular}
\end{table}
\fi


\vspace{5pt}
\subsection{Discussion}
\vspace{10pt}
\subsubsection{Effectiveness of Circuit Transformation}%~\newline
% \vspace{-5pt}

DeepGate uses the logic synthesis tool to transform the circuits from different sources into unified AIG forms. One may wonder the performance of DeepGate if the network is directly trained on the original circuits, wherein other gate types (e.g., XOR, NAND, NOR, and OR) are also included. To investigate the effectiveness of the circuit transformation in DeepGate, we conduct the controlled experiments on EPFL and IWLS benchmarks, as shown in Table~\ref{tab:epfl}. 

Take EPFL as an example, we extract $375$ sub-circuits from the original designs, and develop two versions: the ones with the original $6$ gates types and the other with AIG transformation. For each version, we train the DeepGate model from scratch. The only difference is that for the former version of the dataset, we assign $7$-d one-hot encoding for the node feature $\mathbf{x}_v$. As can be observed from Table~\ref{tab:epfl}, DeepGate trained on AIGs performs better than the one trained on the original circuits by a large margin ($33.94\%$ relative prediction error reduction on EPFL). The same observation can be obtained from the results on IWLS circuits. 

Such improvements originate from the benefit of circuit transformation because when only two logic gate types are considered, representation learning difficulty is reduced dramatically without any impact on circuit functionalities. Also, we manually check the usage frequency of different gate types in the original formats, and observe that some gates types (e.g., XOR and NAND) are used much less frequently. Such in-balanced gate distributions may lead to insufficient training, causing higher prediction errors. 

Additionally, we directly apply the pre-trained DeepGate model on the merged AIG dataset, as shown in Section~\ref{sec:dataset} for comparison. As can be observed, DeepGate trained on the dataset consisting of different benchmarks can further reduce the prediction errors by $51.37\%$. It supports the claim that unifying different circuit designs into a common intermediate representation can help the model learn a better representation of logic gates.


\begin{table}[t!]
\centering
\caption{The Performance of DeepGate with and without Circuit Transformation} \label{tab:epfl}
\begin{tabular}{@{}lccc@{}}
\toprule
  & w/o Tran. & w/ Tran.    & Pre-trained \\ \midrule
 EPFL & 0.0442     & 0.0292 & 0.0142        \\ 
 IWLS & 0.0447     & 0.0342 & 0.0209        \\
 \bottomrule
\end{tabular}
%\vspace{-10pt}
\end{table}


\vspace{10pt}
\subsubsection{Impact of Recurrence Iterations}%~\newline
% \vspace{-5pt}

During the inference phase, the number of iterations $T$ can be set as different values. The higher the value, the higher the computational cost. % instead of the one used in training. In previous experiments, $T$ is fixed as $10$. 

We enumerate different values for $T$, ranging from $1$ to $50$. We observe that our GNN model is able to decrease the prediction loss as $T$ increases. However, the prediction error converges quickly at around $T=10$, despite the circuit size. Such experimental results further demonstrate the scalability of the proposed DeepGate solution. 
%This indeed shows the important property of DeepGate again: scalability. Consequently, the computational cost will not be an issue when we apply the model for large-scale circuits. 

==> dac22/intro.tex <==
\vspace{5pt}
\section{Introduction}
\label{sec:intro}
\vspace{5pt}

The rise of deep learning (DL) has aroused much interest in applying it to solve various electronic design automation (EDA) problems that otherwise rely on some heuristics or hand-engineered rules, as surveyed in~\cite{huang2021machine}. The most natural representation of circuits and netlists is a graph. With the recent success of graph neural networks (GNNs)~\cite{kipf2016semi,hamilton2017inductive} in modeling non-structured data, various works have explored its potential on EDA problems such as congestion prediction~\cite{kirby2019congestionnet} and testability analysis~\cite{ma2019high}. These works focus on learning a particular function that takes the circuit graph as input and directly maps it to output for desired EDA tasks, without considering the internal computational process in the circuits. 

Recently, a notable trend in the deep learning community is to employ pre-trained models for many downstream tasks rather than learning a specific model for each task from scratch~\cite{han2021pre}. For example, a series of convolutional neural networks (CNNs) are pre-trained on the ImageNet dataset~\cite{krizhevsky2012imagenet}. They perform well on other computer vision (CV) tasks such as image segmentation~\cite{minaee2021image} and object detection~\cite{ren2015faster} by fine-tuning with a small amount of task-specific data. Similarly, pre-trained Transformer-based language models (e.g., GPT~\cite{brown2020language} and BERT~\cite{devlin2018bert}) have achieved unparalleled performance on various natural language processing (NLP) tasks.

Whereas in the EDA domain, despite all the recent efforts in learning-based solutions~\cite{huang2021machine}, obtaining a \textit{general and effective circuit representation} that serves as the basis for solving various EDA tasks has not been addressed yet. In this work, we take the first step towards this direction by introducing a novel GNN-based solution for the representation learning of logic gates, namely \textit{DeepGate}, which is aware of the logic computation procedure and the structural information of combinational circuits.

Naturally, logic circuits can be modeled as directed acyclic graphs (DAGs), in which logic gates appear in a specific topological order. Therefore, one could collect many logic circuits and resort to existing DAG-GNN architecture~\cite{zhang2019dvae,thost2021directed} to learn the node embedding for each logic gate with some supervision tasks (e.g., Boolean satisfiability~\cite{amizadeh2018learning}). However, we argue that such straightforward solutions cannot effectively extract information from circuit graphs. 


Firstly, logic circuits could follow different design styles and use diverse technology libraries containing various logic gate types, leading to heterogeneous circuit graphs with mixed distributions that are challenging to learn. In DeepGate, we propose to conduct learning on a general intermediate representation of logic circuits, i.e., \textit{and-inverter graph} (AIG), with the help of logic synthesis tools~\cite{brayton2010abc}. The benefits are twofold: (i). Such a unified format constrains the circuit graph distribution without changing circuit functionalities. All the transformed circuits only feature two types of logic gates (i.e., 2-input AND gate and inverter); (ii). The logic synthesis procedure naturally introduces a strong inductive bias of practical circuits for effective learning with GNN models.

%To solve this issue, we take advantage of logic synthesis tools and adopt a general internal representation of circuits, i.e., And-Inverter Graph (AIG)~\cite{mishchenko2006dag} to unify the format of circuits, which serve as the foundation for effective learning. % This approach is consistent with the fact that practical circuits are always optimized for timing and power. 

Secondly, the effectiveness of representation learning heavily relies on supervision tasks. For example, when pre-training CV models, the image class labels of the ImageNet dataset serve as the cornerstone. In contrast, considering the difficulty in annotating a textual dataset as large as ImageNet, self-supervised tasks are used instead in NLP pre-trained model development. For effective circuit representation learning, we propose to use the signal probability (i.e., the probability of being logic ‘1’) for every node as rich supervision because it embeds the genuine logic relationship of each node in the circuits. To be specific, we perform logic simulations with a large amount of random patterns to obtain faithful probability values for supervision.

Last but most important, existing GNN models are general solutions designed to extract information from all kinds of graphs, while circuit graphs are a unique type of graph with logic relationships between nodes. In this work, we design a dedicated GNN model for circuit graphs, significantly enhancing the learning effectiveness. 

We summarize the contributions of this work as follows:
 
\iffalse
DeepGate uses gate type as the only input feature vector for each node %whereas the previous DL based EDA solutions require different node and edge attributes to solve a particular problem ~\cite{kirby2019congestionnet, pmlr-v97-zhang19e} 
and learns a meaningful circuit representation. It predicts the logic probabilities for every node in circuit that approximates the probabilities achieved through logic simulation. %Due to accuracy in probabilities prediction, DeepGate can be applied to many EDA tasks that relies on logic probabilities.
%We evaluate the effectiveness of DeepGate on \textit{Test Point Insertion} problem where the DeepGate prediction guides about the location of desired test points and outperforms statistical approach \cite{Brglez1984OnTO} that fails at reconvergent nodes. 
We summarize the contributions of this work as follows:
\fi
\begin{itemize}
    \item To the best of our knowledge, DeepGate is the first work for the \textit{general and effective circuit representation learning} problem. Specially, we propose a novel design flow to tackle this problem: (i). circuit transformation in AIG form; (ii). supervision with logic-simulated probabilities; (iii). representation learning with a dedicated GNN model for circuit graphs. 
    \vspace{5pt}
    \item We propose a novel GNN model for circuit graphs that exploits unique circuit properties, including \textit{attention mechanisms} that mimic the logic computation procedure and \textit{reversed propagation layers} that consider logic implication effects.
    \vspace{5pt}
    %i) Model the circuits as DAG. ii) Optimized the circuits before training by doing logic synthesis.  %2) Add the reconvergence structures in circuit as the domain knowledge for GNN and propose two methods i) Modified Attention Mechanism and ii) Skip Connection to deal with it.3) Optimized the circuits before training by doing logic synthesis
    %\item  Novel DeepGate architecture that exploits logic simulation results as supervision and contains unique back propagation for circuits
    %\item We exploit the reconvergence area in circuit as the domain knowledge for GNN and propose two methods 1) a custom Attention based aggregator 2) Skip Connection to deal with it. This remarkably increases the performance of our method for complex structures of circuits.
   %  with the help of DAG-GNN architecture and uses gate type as the only node feature vector for effective representation learning. 
    \item Reconvergence structures are inevitable due to logic sharing in multi-level logic networks, and they are the main challenges for logic analysis~\cite{roberts1987algorithm}. We treat them as first-class citizen and introduce novel solutions in our GNN model. 
    %We use logic simulated probabilities as the rich supervision as it contains the true execution behaviour of logic circuit and effectively reveal many circuit properties %. It helps to achieve the goal of learning computations embedded in the circuits.
    % \item In addition to forward propagation layer, DeepGate also uses a novel reverse propagation layer that keeps the original signal traversal intact in the underlying circuit.
    %\item For the first time, we explore a way of reverse information propagation mechanism in GNN that exactly mimics the logic computation and signal traversal procedures of circuits.
    %\item DeepGate uses 2-layer (one forward and one backward) recursive model in which reverse layer is customized to mimic the original signal propagation in the underlying circuit.
    %\item A novel DL model for circuits that uses gate type as the only input feature vector for effective representation learning.
    %\item An effective DL model that approximate logic simulation probabilities in less time and outperform the existing TPI solutions.
\end{itemize}

We learn the representations of logic gates with many small subcircuits extracted from benchmark circuits. Experimental results performed on large circuits show the efficacy and generalization capability of DeepGate. We organize the remainder of this paper as follows. We review related works in Section~\ref{sec:related}. Section~\ref{sec:method} introduces the DeepGate architecture, while in Section~\ref{sec:experiment}, we present the experimental results on various circuits. Finally, Section~\ref{sec:conclusion} concludes this paper.





%as shown in Figure~\ref{FIG:RC}. 
%They are also enriched with structural information such as reconvergence fanoutsthat requires special processing. We propose to process the reconvergence fanouts as a special structure using \textit{Skip Connection}.


\iffalse
This kind of approach lacks modeling the inductive bias present in the circuit that helps in learning a meaningful circuit representation using GNNs. Naturally, circuits are directed acyclic graphs (DAGs) but many works represent the circuits as undirected graphs \cite{kirby2019congestionnet,ma2019high}. Besides this, logic circuit follows a computational-aware design in which gates appear in a specific topological order. They are also enriched with structural information such as reconvergent fanouts that requires special processing. Existing works do not take advantage of such inductive biases present in the circuits despite the DAG-NN architecture used in \cite{pmlr-v97-zhang19e}. Moreover, in the existing DL based EDA works, supervision is usually given by commercial EDA tools~\cite{ma2019high} for a specific EDA task that set a sub-optimal upper-bound in learning.

%However, most of these works focus on learning a function which  maps each input to a particular output. Such kind of function modelling does not care about learning the actual internal computational process. Whereas logic circuits follows a computational aware design, and are enriched with structural information such as reconvergent fanouts. There are other inductive biases present in circuit such as circuits are directed acyclic graphs (DAGs), exhibit the pattern of long-term dependency between internal nodes and are optimized for timing and/or power. These factors induce a significant bias in real circuit designs that helps in learning a good circuit representation. Existing works do not take advantage of such inductive biases present in the circuit despite the DAG-NN architectre used in [18].

  % For example, inserting a NOT gate before one internal node can easily change the original computation, and results in total different logic.
%They also exhibit the pattern of long-term dependency between internal nodes (in form of reconvergence fanouts). \cite{zhang2019dvae} proposed a framework to learn computations on DAG but they do not consider the long term dependencies between nodes. 

%In this work, we focus on learning  a good circuit representation that is aware of internal computational process as well as structural information in combinatorial circuits. Learning computations will give us the semantics of how systematically the information is processed internally at each node in the graph. As, logic simulation reflects the true computational behaviour at all gates in the circuits. So, we consider a more basic and fundamental problem: \textit{can a neural network learn to mimic the logic simulation?} and to achieve this, we use logic simulation based probabilities as a rich supervision signal for each node in the DAG. Besides the rich supervision, we also explore many inductive biases present in the logic circuits such as reconvergence fanouts and also reverse propagation scheme for neural models based on circuits, while keeping the signal propagation intact in underlying circuit. This helps to learn the long term dependencies between nodes, consequently the overall structure of the circuit, We add these informations as the domain knowledge to our framework and propose a custom GNN model, named \textit{DeepGate} to encode it.


Considering the limitations in prior works, we focus on learning a good circuit representation that is aware of internal computational process as well as enriched with the structural information in combinatorial circuits. In this work, we propose \textit{DeepGate}, a novel DL model that is capable of exploiting the relational inductive bias in circuits. For this purpose, we model the circuit as directed graph, use DAG-GNN architecture to aggregate the information while following the topological ordering of logic gates and process the reconvergence fanouts as a special structure using \textit{Skip Connection} %and \textbf{2) Modified Attention Mechanism}. 
Practical circuits are optimized for timing and/or power, inducing significant bias in real circuit designs. So, before training we optimized the circuit dataset by doing logic synthesis to introduce such bias in the dataset. 

DeepGate uses 2 layer recursive model  for information propagation that contains one forward and one reverse layer. %While the reverse signal propagation is non trivial in the circuit. So, we propose a customized reverse layer that keeps the original signal propagation intact in underlying circuit.
Besides the inductive bias modelling, supervision is another factor that affect the learning of a DL model. In this project, we use the logic simulated probability (i.e., the probability to be logic ‘1’ in the circuit) for every node as supervision because it embeds the logic relationship of each node in the circuits and also, for reconvergence fanouts, logic simulation is arguably the only way to obtain the actual value for such structures.


%We also propose a novel recursive message passing scheme in which the reverse layer keeps the original signal propagation intact in underlying circuit. For a particular, logic gate \(v\) in circuit, the logic value of its successor gate \(u\) is also related to the side-inputs of \(u\). Consequently, we propose to design the reverse layer in which the hidden state of each node is updated by aggregating features with one of its successors and the successor's side-inputs.



%A rich supervision reveals many properties of data. In this project, we use the logic simulated probability (i.e., the probability to be logic ‘1’ in the circuit) for every node as supervision, which satisfies the following requirements: (i) It embeds the logic relationship of each node in the circuits (ii). Reconvergence structures makes the circuit analysis challenging and logic simulation is arguably the only way to obtain the actual value for such structures; (iii). The logic probability of each gate itself plays an essential role in many EDA tasks.


%\textbf{Problem definition: }More formally, given a combinatorial circuit \- a DAG representation \- with different gate types, the probability prediction is the task of producing probability values for all nodes that matches the logic probabilities obtained from logic simulations (\textit{i.e., }feed large amount of inputs into the circuit and observe the chances of nodes being $1$). In order to go from a combinatorial circuit to accurate probability estimations for all gate nodes, an algorithm has to be equipped with a number of capabilities, such as mimicking the logic computational behaviours, capturing the long-term dependency between \textit{fan-in} (\textit{i.e., }reconvergence). 

DeepGate uses gate type as the only input feature vector for each node whereas the previous DL based EDA solutions require different node and edge attributes to solve a particular problem ~\cite{kirby2019congestionnet, pmlr-v97-zhang19e}.  and learns a meaningful circuit representation. It predicts the logic probabilities for every node in circuit that approximates the probabilities achieved through logic simulation. Due to accuracy in probabilities prediction, DeepGate can be applied to many EDA tasks that relies on logic probabilities. We evaluate the effectiveness of DeepGate  on \textit{Test Point Insertion} problem where the DeepGate prediction guides about the location of desired test points and outperforms statistical approaches \cite{Brglez1984OnTO} and \cite{goldstein1980scoap} that fails at reconvergent nodes. %as shown in Figure~\ref{FIG:RC}. 

\iffalse
\begin{figure}[h]
	\centering
	\includegraphics[width=0.5\linewidth]{dac22/figs/Wrong_COP.pdf}
	\caption{This figure shows the inaccurate results of COP~\cite{Brglez1984OnTO} on a reconvergent node. The actual probability of logic-1 is 0\% but COP gives the 25\%.}
	\label{FIG:RC}
\end{figure}
\fi
%We apply the learned representation from DeepGate to a downstream EDA application \textit{Test Point Insertion}. Currently, Logic simulation is used as a testability analysis tool to guide the TPI Problem. But it is a costly procedure  because for large circuits, huge amount of patterns are required to be simulated to achieve the accurate results. 

%To avoid this, \cite{Brglez1984OnTO} and \cite{10.1145/800139.804528} proposed solution based on hand-engineered rules for different gate types to get the testability analysis. But these approaches neglect the reconvergent structures in circuits, the obtained probability predictions are usually inaccurate for reconvergent nodes, misguide about the test point locations and results in unsatisfactory circuit behaviours. Our experimental results shows that DeepGate is able to approximate logic simulation results within less time and cost, outperforms \cite{Brglez1984OnTO} and \cite{10.1145/800139.804528} and come up with more feasible test points locations.

\fi




%Our proposed framework is capable to learn a generic circuit representation that could be applied to various circuit based downstream tasks. We explore SAT problem as one of the downstream task and our experimental results shows that our approach outperforms the existing learning based SAT solutions.



==> dac22/method.tex <==
\vspace{10pt}
\section{Proposed Solution}
\label{sec:method}

%{\color{red}In this section we formally define the DeepGate, a DAG-NN based model for circuit representation learning. DeepGate is a novel recursive information propagation model that explicitly exploits the inductive bias present in logic circuits and uses a custom message passing between nodes to encode the underlying circuit structure and its properties. 
%}

\begin{figure*}[t!]
	\centering
	\includegraphics[width=\linewidth]{dac22/figs/Architecture.pdf}
	\caption{The Overview of DeepGate.} %(a) shows the data preparation process. (b) shows the DeepGate model for circuit representation learning}
	\label{FIG:Arch}
\end{figure*}


\subsection{Overview of DeepGate}

Figure~\ref{FIG:Arch} presents the overview of the proposed DeepGate solution, consisting of two stages for the neural representation learning of logic gates: 

\begin{itemize}
    \item \textbf{Circuit Data Preparation:} Given a pool of circuit designs, we use logic synthesis tools to transform them into a unified AIG format. We then perform logic simulations on the circuits with sufficient random patterns to obtain the signal probability (i.e., the probability of node being logic `1`) on every node as supervision. We elaborate the details in Section~\ref{sec:data-pre}.
    \vspace{5pt}
    \item \textbf{Probabilities Prediction with DeepGate:} Given a circuit dataset and the logic-simulated probabilities as the supervision task, we introduce a novel GNN model dedicated for circuit graph analysis to learn the neural representations of logic gates, as detailed in Section~\ref{sec:model}.
\end{itemize}


\subsection{Circuit Data Preparation}\label{sec:data-pre}
Some circuits are at the register-transfer level, while others are gate-level netlists mapped with various libraries. Such heterogeneity across circuits is a challenge for GNN model development. To tackle this problem, we resort to the logic synthesis tool ABC~\cite{brayton2010abc} and transform all circuits into the unified AIG format. If the original circuit is too large, we extract small sub-circuits with circuit sizes ranging from $30$ to $3k$ gates. Note that, we test the effectiveness of DeepGate on much larger circuits for its generalization capabilities.

The benefits of such circuit pre-processing flow include: (i).~Only two logic gate types (i.e., 2-input \textit{AND} gate and 1-input \textit{Not} gate) are considered, which would dramatically reduce representation learning difficulty; (ii).~Applying logic synthesis introduces strong relational inductive bias into the resulting circuit graphs; (iii).~The constraint on circuit size facilitates efficient GNN training with both reduced sizes of circuit graphs and less time for preparing supervision labels. 

There are many possibilities to annotate a circuit, e.g., the satisfiability of the circuit~\cite{amizadeh2018learning}. However, a good supervision task should satisfy the following condition: the labels should be easily obtained while retaining rich information for both the logic function and the structural information of the circuits. In DeepGate, we propose to use the signal probability on every node as supervision, which satisfies the above requirements: (i). It is relatively easy to obtain highly-accurate probability values by running logic simulations on many random input patterns, especially when the circuit size is limited; (ii). A unique yet important property of logic circuits that makes circuit analysis challenging is the reconvergence structures, and logic simulation is arguably the only way to obtain the actual value for such structures; (iii). The logic probability of each gate itself plays an essential role in many EDA tasks. 

\subsection{GNN Model in DeepGate}\label{sec:model}

Given circuit graphs in AIG form, the objective of our GNN model is to estimate the probability of every node such that it would be as close to the genuine signal probability as possible. 
%To learn the accurate probability prediction, we propose DeepGate, in which circuit graph information is processed sequentially from source nodes to sink nodes %similar to \cite{thost2021directed,zhang2019dvae}, but in the recurrent manner. It simulates how a logic inference of circuits is really performed -- we do the logic calculation from PIs to POs sequentially.  
Different from existing DAG-ConvGNNs~\cite{thost2021directed,zhang2019dvae} and DAG-RecGNNs~\cite{amizadeh2018learning} models that focus on learning the topological information in the graph, 
%graph level representation and do not consider the specific properties in circuits,  whereas 
DeepGate is designed to learn 
%node level representation for circuit graphs. Equipped with dedicated model design, it learns 
both the circuit structural information and the computational behaviour of logic circuits, and embed them as vectors on every logic gate.

We now elaborate on the detailed GNN model design in DeepGate. Given a circuit graph $\mathcal{G}$, we embed the gate type of each node $v$ with one-hot encoding in $\mathbf{x}_v$. To be specific, as only primary inputs (PIs), \textit{And} gates and \textit{Not} gates are present in AIGs, we assign a $3$-d vector for each node according to its gate type. It should be noted that instead of relying on the probability-based measurements in previous works~\cite{zhang2020grannite,ma2019high}, our model only requires gate type information for the representation learning. We also have hidden states $\mathbf{h}_v$ %\footnote{$\mathbf{h}_v$ can have the superscript $t$ to indicate the current iteration} 
for every node, which is initialized randomly. Given these, DeepGate resorts to attention-based aggregation design~\cite{thost2021directed,velikovi2017graph} and the gated recurrent unit (GRU)~\cite{zhang2019dvae} as the update function.

\vspace{5pt}
\textit{Aggregation.} We use the attention mechanism in the additive form to instantiate the AGGREGATE function in Equation~\eqref{eq:dag-edge}, wherein the aggregated message $\mathbf{m}_v^t$ for a node $v$ at $t^{th}$ iteration is computed by:
\begin{equation}
\small
    \mathbf{m}_v^t = \sum_{u \in \mathcal{P}(v)}  \alpha_{uv}^t  \mathbf{h}_u^t
\text{\quad where\quad} \alpha_{uv}^t = \mathop{softmax}\limits_{u \in \mathcal{P}(v)} (w_1^\top \mathbf{h}_v^{t-1}+ w_2^\top \mathbf{h}_u^t)
\label{eq:attn}
\end{equation}
where $\alpha_{uv}^t$ is a weighting coefficient that is computed by following the query-key design as in usual attention mechanisms. To be specific, $\mathbf{h}_v^{t-1}$ serves as \textit{query}, and representation of predecessors from current iteration $t$, $\mathbf{h}_u^t$, serves as \textit{key}. The intuition behind using the attention mechanism for aggregation is that when we do the logic computation in digital circuits, the controlling value of a logic gate determines the output of that gate. Therefore, controlling values are far more important than non-controlling values. To mimic this behaviour, the attention mechanism can learn to assign high weights for controlling inputs of gates and give less importance to the rest of the inputs.

\vspace{5pt}
\textit{Combine.} We then use the GRU to instantiate the COMBINE function for updating the hidden state of target node $v$:
\begin{equation}
    \mathbf{h}_v^t = GRU([\mathbf{m}_v^t,\mathbf{x}_v], \mathbf{h}_v^{t-1})
\end{equation}
wherein $\mathbf{m}_v^t$, $\mathbf{x}_v$ are concatenated together and treated as input, while $\mathbf{h}_v^{t-1}$ is the past state of GRU. 

On the one hand, DeepGate adopts the recursive DAG-GNNs functional defined in Equation~\eqref{eq:recdag-edge}.
The reasons for using the recurrent architecture are two-fold: (i). 
%as the supervision comes from many logic simulation runs, 
it is unrealistic for GNNs to capture the circuit's functional and structural information with a single forward propagation; (ii). the recurrent learning procedure facilitates reaching stabilized node embeddings quickly. 
%The experimental results demonstrated in Section~\ref{sec:prob} also prove the correctness of this model choice. 


On the other hand, our proposed GNN model differs from previous DAG-GNNs~\cite{amizadeh2018learning,thost2021directed,zhang2019dvae} that initialize $\mathbf{h}_v^0$ as $\mathbf{x}_v$ and treat the aggregated message as the state of recurrent function. In contrast, we fix the gate type information of nodes $\mathbf{x}_v$ as inputs for all iterations. Such employment can avoid the information vanishing of gate properties during the long-term recursive propagation. 


\vspace{5pt}
\textit{Reversed Propagation Layer.}
In DeepGate, we also consider backward information propagation, i.e., processing the graph in reversed topological order. One of the main reasons to introduce the backward layers in our framework is that logic implication and backtracking in the reversed order can be highly useful for predicting the states of nodes. It also helps stabilize training, as proved in sequence-to-sequence learning tasks~\cite{sutskever2014sequence}. 


\vspace{5pt}
\textit{Regressor.} After $T$ iterations, we pass the hidden states of nodes $\mathbf{h}_v^T$ into a multi-layer perceptron (MLP), which computes a single scalar for every node to regress the simulated probabilities. The weights of MLP are shared for nodes with the same gate types. We train the network to minimize the \textit{L1} loss between the prediction $\hat{y}_v$ and the true probability $y_v$.


\begin{figure}[t!]
 	\centering
 	\includegraphics[width=0.8\linewidth]{dac22/figs/SC.pdf}
	\caption{Information Propagation at Reconvergence Node using Skip Connection}	\label{fig:SC}
	\vspace{-5pt}
\end{figure}

\subsection{Skip Connection for Reconvergence Structure with Positional Encoding}
In the previous section we have described the core components of DeepGate necessary for predicting the logic probabilities of nodes. However, the logic inference on reconvergence nodes is different from normal nodes and such structures are inevitable due to logic sharing in multi-level logic networks. Hence, they are the main challenge for logic probability analysis. %~\cite{roberts1987algorithm}.
To accommodate their impact, we introduce the improvement into DeepGate to enable special processing for reconvergence nodes as shown in Figure~\ref{fig:SC}. 

Firstly, we maintain the information of reconvergence nodes during circuit data preparation, including its corresponding source fan-out node, and the logic level difference between the source nodes and reconvergence nodes. Secondly, we add direct edges between the fan-out node and the reconvergence node, named \textit{skip connection} here. The new edges facilitate the information exchange from fan-out nodes to reconvergence nodes. Last but not least, we leverage the positional encoding technique~\cite{vaswani2017attention} to differentiate the skip connection and the normal connection. To be specific, the function $\gamma(D)$ is a mapping of logic level difference $D$ between source fan-out node and reconvergence node into a higher dimensional space $\mathbb{R}^{2L}$:
\begin{equation}
    \footnotesize
    \label{eq:positional}
    \gamma(D) = (\sin(2^0\pi D), \cos(2^0\pi D), \cdots, \sin(2^{L-1}\pi D), \cos(2^{L-1}\pi D))
\end{equation}
The impact of the fanout node on the reconvergence nodes depends upon the distance between them. Generally speaking, the longer the distance is, the lesser impact it has on the reconvergence node. The above function can induce the knowledge of how much fanout node can impact the result of reconvergence node into the model. We assign the encoded vector as the edge attributes to skip connection and incorporate it into the coefficient calculation described in Equation~\eqref{eq:attn} as the third input. %{\color{red}For the normal edges, we assign $1$ as the input to the positional encoding function to obtain their edge attributes. }


% \begin{algorithm}[!h]
% \caption{Add Skip Connection} \label{Algo:ASC}
% \KwIn{Circuit graph i.e., nodes and edges array ($x$, $edge\_index$). reconvergent node list $RCN$ and source fanout node list of reconvergent nodes $SFN$}
% \KwOut{Updated circuit edges with positional encoding and skip connection ($updated\_edge\_index$) }

% $updated\_edge\_index$ = add\_positional\_encoding($edge\_index$,$1$)

% \For {$i \leftarrow 0$ \KwTo $length(x)-1$} {
%         \If {$x[i]$ exists in $RCN$} {
%              $s$ = get\_source\_node($x[i]$, \ $SFN$)\;
%             $ll\_diff$ = get\_logic\_level\_difference($x[i]$, \ $x[s]$)\;
%             $new\_edge$=create\_new\_edge($i$, $s$)\;
%             $updated\_edge$=encode\_new\_edge($new\_edge$, $ll\_diff$)\;
%             $updated\_edge\_index$=update\_edges($updated\_edge\_index$, $updated\_edge$)
%         }
% }
% \BlankLine
% \end{algorithm}

%  \begin{figure}[t!]
% 	\centering
% 	\includegraphics[width=0.5\linewidth]{dac22/figs/RC_Solutions.pdf}
% 	\caption{Information Propagation at Reconvergent Node using Skip Connection}
% 	\label{fig:SC}
% \end{figure}

==> dac22/related.tex <==

\section{Related Works}
\label{sec:related}
\vspace{5pt}



\begin{figure}[t!]
	\centering
	\includegraphics[width=0.8\linewidth]{dac22/figs/DAG.pdf}
%	\vspace{-5pt}
	\caption{The Circuit Representation as DAG}
	\label{FIG:DAG}
 %	\vspace{-5pt}
\end{figure}


\subsection{Graph Neural Networks}
%To facilitate graph analysis with DL techniques, 
Graph neural networks~\cite{hamilton2017inductive,kipf2016semi} have received a lot of attention for their effectiveness in modeling non-structured data. By learning vectorial representations on graphs via feature propagation and aggregation, GNNs show convincing results in various domains~\cite{hu2020open,gilmer2017neural, wu2018socialgcn}. The most popular GNN model employs a message-passing neural network architecture, which computes representation/hidden states $\mathbf{h}_v^\ell$ for node $v$ in a graph $\mathcal{G}$ at every layer $\ell$ and a final graph representation $\mathbf{h}_\mathcal{G}$, as in \cite{gilmer2017neural}: 
\begin{equation}
\hspace{-1mm}
    \footnotesize
    \mathbf{h}_v^\ell = \text{COMBINE}^\ell(\mathbf{h}_v^{\ell-1}, \text{AGGREGATE}^\ell(\{\mathbf{h}_u^{\ell-1} | u\in \mathcal{N}(v)\})), \ell = 1,.,L
    \label{eq:gnn-edge}
\end{equation}
\begin{equation}
    \small
    \mathbf{h}_\mathcal{G} = \text{READOUT}(\{\mathbf{h}_v^L, v\in \mathcal{V}\})
    \label{eq:gnn-graph}
\end{equation}
wherein $N(v)$ denotes neighboring nodes of node $v$ and $L$ is the number of layers. The parameterized function $\text{AGGREGATE}^\ell$  aggregates messages from neighboring nodes $N(v)$, and $\text{COMBINE}^\ell$ obtains an updated hidden state after aggregation. Finally, the function $\text{READOUT}^\ell$   retrieves the states of all nodes $\mathcal{V}$  and produces the graph neural representation. A notable GNN architecture is the graph attention network (GAT) \cite{velikovi2017graph} that considers the importance of different neighbors during aggregation.

Directed acyclic graphs (DAGs) are a special type of graphs, yet broadly seen across many domains, including circuit modeling (see Fig.~\ref{FIG:DAG}). Recently, few studies have been dedicated to DAG-GNN designs~\cite{zhang2019dvae,thost2021directed}, which propagate the message following the topological ordering between nodes and only consider the predecessors in the $\text{AGGREGATE}^\ell$ function, as demonstrated in Equation~\eqref{eq:dag-edge}.
\begin{equation}
\hspace{-0.5mm}
    \footnotesize
    \mathbf{h}_v^\ell = \text{COMBINE}^\ell(\mathbf{h}_v^{\ell-1}, \text{AGGREGATE}^\ell(\{\mathbf{h}_u^{\ell} | u\in \mathcal{P}(v)\})), \ell = 1,...,L
    \label{eq:dag-edge}
\end{equation}
The major difference between Eq.~\eqref{eq:dag-edge} and Eq.~\eqref{eq:gnn-edge} is that in DAG-GNN, the aggregation function for $v$ will be only executed after all of its predecessors' hidden states have already been computed.
 
 Besides stacking $L$ layers to increase the depth of the network, one can also apply the same model for $T$ times in the \textit{recurrent} fashion to generate the final embedding~\cite{ amizadeh2018learning}:
\begin{equation}
    \footnotesize
    \mathbf{h}_v^t = \text{COMBINE}(\mathbf{h}_v^{t-1}, \text{AGGREGATE}(\{\mathbf{h}_u^{t} | u\in \mathcal{P}(v)\})), t = 1,...,T
    \label{eq:recdag-edge}
\end{equation}

Using the taxonomy defined in~\cite{wu2020comprehensive}, we name the two variants of DAG-GNNs described in Equations~\eqref{eq:dag-edge}--\eqref{eq:recdag-edge} as \textit{DAG-ConvGNNs} and \textit{DAG-RecGNNs}, respectively.

\iffalse
\begin{figure}[t!]
	\centering
	\includegraphics[width=1\linewidth]{figs/gnn-dagnn.pdf}
	\caption{Information Propagation in conventional GNNs and DAG-GNNs.} %a)Every node is aggregating information only from its predecessors in a sequential manner. b)All nodes are aggregating information from all their neighbors simultaneously.}
	\label{fig:eda_gnn_flow1}
\end{figure}
\fi
%There are some more recent works that involved formulating neural model on directed and undirected graph \textit{e.g.}, \cite{li2017gated,shuai2015dagrecurrent}. The former proposed a deep model that performs GRU updates in iterative manner on undirected graphs while the latter proposed a framework that performs RNN like updates on underlying directed graphs. \cite{thost2021directed} consider partial ordering between nodes in DAG as inductive bais and  proposed a topological batching scheme in which information is processed according to flow define by partial order. 

\iffalse
\subsection{Neuro-Symbolic Computing}
{
\color{red}
Introduce the structure they used. There's a survey paper~\cite{lamb2020graph} we can refer to. Also a GNN survery~\cite{wu2020comprehensive} can be referred. Some following works related to \textit{RecGNN} defined in~\cite{wu2020comprehensive} is listed in the \textit{bib} file.

NeuroSAT, CircuitSAT and other models for to solve combinatorial optimization. They consider one of the NP-complete problems: propositional satisifiability (SAT) problem. Advantage: good generalization ability to out-of-sample problems. Drawback: the performance is worse, and the computational cost is quite expensive.

Even though the structure we used is quite similar to theirs, but the basic tasks we deal with has nothing in common. So we can easily differentiate our work from theirs.
}

The effectiveness of deep learning models has paved its way to classical computer science where many combinatorial optimization problems are explored as its applications. For instance, \cite{dai2018learning} uses GNN model to learn embeddings of graphs and used these embeddings to learn the search heuristics in NP complete Minimum Vertex Cover (MVC), Maximum Cut and Traveling Salesperson (TSP) problems. \cite{NEURIPS2019_12e59a33} also follows similar approach and learns a heuristics to solve boolean satisfiability problem using GNN. \cite{li2018combinatorial} also used GCN as a heuristic to search problem and apply this method on four canonical NP-complete problems, Maximal Independent Set, MVC, Maximal Clique, and the Boolean Satisfiability Problem (SAT)

\fi
\subsection{GNN-Based Solutions for EDA Problems}
Existing GNN-based EDA solutions use an end-to-end flow for specific EDA tasks wherein the labels are usually extracted from commercial EDA tools. 

To the best of our knowledge, the first GNN-based EDA technique is applied to the test point insertion (TPI) problem, which is formulated as a node binary classification problem and solved with a graph convolutional network~\cite{ma2019high}. 
%in which they learn different weights for successors and predecessors during aggregation. 
The ground-truth labels are collected from commercial TPI tools, revealing whether a particular node is "easy to observe" or not. CongestionNet~\cite{kirby2019congestionnet} models the circuit as an undirected graph and trains a GAT model to predict the congestion of the final physical design on a per-cell basis. 
%Nodes are represented by cell types, sizes, pin counts, and logic descriptions. To get the ground truth labels for the nodes, congestion mapsobtained after placement and routing are split into grids. The congestion value of each grid is taken as a label for the cells that were placed into that grid. 
GRANNITE~\cite{zhang2020grannite} conducts power estimation using a DAG-GNN model. Gate netlists are mapped onto graphs with per-node (gate) and per-edge (net) features. They achieved good accuracy (less than 5.5\% error across a diverse set of benchmarks) for fast (<1 second) average power estimation on designs up to 50k gate. 
%There is another GNN-based EDA solution proposed in the literature \textit{i.e.}, placement and route
Recently, \cite{xie2021net} proposes a GAT-based model named \(Net^2\) for pre-placement net length estimation. 
%To that end, the authors model the netlists as directed graphs, where nets represent nodes, and edges connect nets in both directions. Node features are the number of cells, fanin, fan-out sizes, and areas. The supervision for nodes is the net length obtained as the half-perimeter wirelength of the bounding box after placement. 
%Specially, a graph is constructed from the netlist, wherein the logic gates are treated as nodes, and the wires between them as edges. 
%To this end, each logic gate is represented with a 4-dimension vector that contains the logic level of each gate, the gate type, and the controllability and observability properties~\cite{goldstein1980scoap}. The ground-truth labels are collected from commercial TPI tools, revealing whether a particular node is "easy to observe" or not. %To learn the embedding from the built graphs, a modified GCN is proposed to aggregate the neighborhood information. The outputs from the proposed model are integrated into testing tools for TPI. 
%Their results show around $11\%$ observation point reduction with the proposed GNN-based solution.

 %The node features are 50-dimension vectors containing information about cell types, sizes, pin counts, and logic descriptions. To get the ground truth labels for the nodes, congestion maps obtained after placement and routing are split into grids. The congestion value of each grid is taken as a label for the cells that were placed into that grid.
\iffalse
CongestionNet~\cite{kirby2019congestionnet} also models the circuit as undirected graphs and trains a GAT \cite{velikovi2017graph} to predict the congestion properties of the final physical design on a per cell basis. Nodes are represented by cell types, sizes, pin counts, and logic descriptions. To get the ground truth labels for the nodes, congestion maps
obtained after placement and routing are split into grids. The congestion value
of each grid is taken as a label for the cells that were placed into that grid. GRANNITE~ \cite{zhang2020grannite} conducts power estimation using a DAG-GNN model for digital designs. Gate netlists are translated into graphs with per-node (gate) and per-edge (net) features. They achieved good accuracy (less than 5.5\% error across a diverse set of benchmarks) for fast (<1 second) average power estimation on designs up to 50k gate. %Results showed that it achieved good accuracy (less than 5.5\% error across a diverse set of benchmarks) for fast (<1 second) average power estimation on designs up to 50k gates.
There is another GNN-based EDA solution proposed in the literature, i.e., placement and route~\cite{xie2021net} that propose a GAT-based model named \(Net^2\) for pre-placement net length estimation.  They represent the netlists as directed graphs, where nets represent nodes, and edges connect nets in both directions. Node features are number of cells, fanin, fan-out sizes,and areas. The supervision for nodes is the net length obtained as the half-perimeter wirelength of the bounding box after placement. Due to the nature of the corresponding EDA problem, it does not learn the neural representations of logic circuits. %, and analog designs~\cite{pmlr-v97-zhang19e}.
\fi
%, such as each gate’s intrinsic state probabilities. GNNs can learn from both graph and input activation features, and likewise GRANNITE learns from both gate-level simulation trace data and input graph (netlist) data. In this way, the model becomes transferable to both new graphs (netlists) and new workloads. .

%The above solutions train separate GNN models for specific EDA tasks from scratch. 
To solve a particular EDA problem, the above techniques typically pre-compute many node/edge features (e.g., SCOAP testability measures in \cite{ma2019high}) %{\color{red} xxx })  
and use existing GNN models to aggregate these features for solution findings. Consequently, the learned node features cannot be transferred among related tasks, despite using the same circuit graphs as inputs. More importantly, an effective representation for circuits should be aware of their logic functions. However, existing solutions ignore it and only consider the structural information in their learning procedure. 

Motivated by the above, we propose to learn a general and effective circuit representation without pre-computing any specific features, as detailed in the following section. 


%even if most of them take the same circuit graph as inputs. Due to the nature of the specific EDA problem, it does not learn the neural representations of logic circuits.
%Consequently, the learned node features cannot be transferred among related tasks. Moreover, the supervision usually comes from commercial EDA tools which set a sub-optimal upper bound for learning process. Last but not the least, data quality has a profound impact on DL model accuracy wherein practical circuits are optimized for timing and/or power that introduce a significant inductive bias in circuit dataset for good model learning. But this aspect is largely ignored by existing solutions. 

%The difference between prior work and our approach is that they focus on solving a specific EDA problem and require many node and/or edge level features instead of learning a generic circuit representation. 

%as they directly train their model on open source benchmarks~\cite{ISCAS89} or some industrial netlists~\cite{ma2019high} . %Also, Except \cite{pmlr-v97-zhang19e}, all existing works model the circuits as undirected graph that is non-trivial in case of logic circuit. 
%These work required  and they do not model the inductive bais from circuit. %Whereas in DeepGate, we learn a circuit representation by considering   %Due to the nature of the corresponding EDA problems, they do notlearn the neural representations of logic circuits and hence are not discussed in detail here. Please refer to the survey paper~\cite{lopera2021survey} for a comprehensive discussion of these techniques. 
%While existing GNN-based EDA solutions have shown some promising results, they suffer from several weaknesses:
\iffalse
\begin{enumerate}
    \item \textit{Lack of inductive bias for circuit modeling}. Circuit graphs are special type of graphs: (i). They are directed acyclic graphs (DAGs); (ii). \emph{Reconvergence} structures are inevitable due to logic sharing in multi-level logic networks~\cite{Mishchenko2006ScalableLS}; (iii). Practical circuits are optimized for timing and/or power. The above properties separate circuit graphs from arbitrary graphs, but they are largely ignored by existing GNN-based EDA solutions. 

    \item \textit{Limited supervision in learning}. In existing solutions, the supervision is usually given by commercial tools for the specific EDA task. On the one hand, these ground-truth labels are often not sufficiently informative for effective learning. For example, for the GNN-based TPI work~\cite{ma2019high}, the only supervision is the binary label on whether each node is easily observable or not provided by commercial tools. On the other hand, such supervision imposes an upper bound on the performance of the learning-based solution.
\end{enumerate}
\fi
